Lightening Anything in Medical Images

The development of medical imaging techniques has made a significant contribution to clinical decision-making. However, the existence of suboptimal imaging quality, as indicated by irregular illumination or imbalanced intensity, presents significant obstacles in automating disease screening, analysis, and diagnosis. Existing approaches for natural image enhancement are mostly trained with numerous paired images, presenting challenges in data collection and training costs, all while lacking the ability to generalize effectively. Here, we introduce a pioneering training-free Diffusion Model for Universal Medical Image Enhancement, named UniMIE. UniMIE demonstrates its unsupervised enhancement capabilities across various medical image modalities without the need for any fine-tuning. It accomplishes this by relying solely on a single pre-trained model from ImageNet. We conduct a comprehensive evaluation on 13 imaging modalities and over 15 medical types, demonstrating better qualities, robustness, and accuracy than other modality-specific and data-inefficient models. By delivering high-quality enhancement and corresponding accuracy downstream tasks across a wide range of tasks, UniMIE exhibits considerable potential to accelerate the advancement of diagnostic tools and customized treatment plans.

==> Sections/Conclusion.tex <==
\section{Conclusion and Future Directions}

This paper presents a novel Diffusion Model called UniMIE, specifically designed for enhancing medical images. Unlike previous approaches, UniMIE does not rely on any training process and instead utilizes a pre-trained model from ImageNet to showcase its unsupervised enhancement capabilities across a wide range of medical image datasets. The effectiveness of UniMIE has been extensively evaluated on three distinct medical image datasets, including corneal confocal microscopy, retinal color fundus, and endoscopy images. The experimental results highlight the superior performance of UniMIE compared to other low-light enhancement methods. Additionally, we have conducted a thorough investigation into the impact of our proposed method on various medical image analysis and clinical tasks, such as nerve segmentation, tortuosity grading, fovea localization, and disease classification.

Given that UniMIE is a training-free method, we plan to integrate it into existing medical equipment, including microscopes and gastroenteroscopes, to further evaluate and validate its practical application. This integration will allow us to assess the effectiveness of UniMIE in real-world medical scenarios and gauge its potential for enhancing medical image quality directly within the existing infrastructure.


==> Sections/Related.tex <==
\section{Related works}

\subsection{Low-light Image Enhancement}

Traditional low-light image enhancement methods can be broadly classified into two categories: histogram equalization (HE) and Retinex-based approaches. However, recent advancements in deep learning techniques have garnered significant attention in this field. For instance, Kin et al.~\cite{lore2017llnet} proposed LLNet, a deep neural network that employs stacked sparse denoising encoders to enhance low-light images naturally. Following this work, Wei et al.~\cite{wei2018deep} curated a dataset consisting of paired low/normal illumination images captured in real-world scenarios (LOL) and devised a novel image decomposition method named Deep Retinex-Net, which demonstrated remarkable light adjustment capabilities based on the Retinex theory. Drawing inspiration from the Retinex theory, KinD~\cite{zhang2019kindling} decomposes the original space into smaller subspaces and incorporates a restoration module to effectively mitigate degradation concealed in dark regions. Expanding on this foundation, KinD++\cite{zhang2021beyond} introduces multi-scale brightness attention, facilitating more adaptive brightness adjustments. In addition to these approaches, LightenNet~\cite{li2018lightennet} predicts the mapping relationship between low-light images and illumination maps, while MBLLEN~\cite{lv2018mbllen} proposes a novel loss function capable of jointly addressing various factors, including brightness, contrast, artifacts, and noise. Furthermore, ExCNet~\cite{zhang2019zero} applies a ``zero-shot'' Exposure Correction Network to estimate suitable ``S-curves'' for backlight images.

To enhance the robustness of image enhancement methods and reduce reliance on data, Guo et al. proposed Zero-DCE~\cite{guo2020zero} in 2020, a lightweight network that is independent of paired or unpaired data. It formulates the LLIE problem as an image-specific curve estimation task. RRDNet~\cite{zhu2020zero}, a Three-branch Convolutional Neural Network, enables illumination adjustment and noise elimination. Yang et al. introduced DRBN~\cite{yang2020fidelity}, a semi-supervised Deep Recursive Band Network, which recovers the linear band representation of enhanced images through supervised learning and improves them through unsupervised adversarial learning. TBEFN~\cite{lu2020tbefn}, a Two-branch Exposure Fusion Network, estimates transfer functions in two branches and refines the enhanced results through fusion. Inspired by the Laplacian pyramid, DSLR~\cite{lim2020dslr} utilizes Multi-Scale Laplacian Residual Blocks to iteratively shift and fuse the original image multiple times, effectively reducing noise and increasing brightness. The weight-sharing self-calibrated illumination learning framework SCI~\cite{ma2022toward} enhances the representational power of individual basic blocks, improves convergence between stages, and achieves enhanced exposure stability with reduced computational burden.


\subsection{Medical Image Enhancement}
In recent years, with the rapid development of image enhancement technology and the increasing recognition of the importance of medical image processing, more and more researchers have conducted relevant studies in this field. Medical image enhancement methods can be categorized into traditional methods and deep learning-based methods. Early medical image enhancement techniques involved adjusting image parameters to enhance low-quality images, such as histogram equalization (HE)~\cite{abdullah2007dynamic}, image contrast normalization (ICN)~\cite{foracchia2005luminosity}, and contrast-limited adaptive histogram equalization (CLAHE)~\cite{setiawan2013color}. Subsequently, based on the Retinex theory~\cite{zhao2020automated}, low-quality images were decomposed into reflectance and illumination components, and prior knowledge was utilized for restoration. However, traditional methods have some evident limitations and may produce unexpected artifacts and structural distortions under complex degradation conditions.

Deep learning-based methods have a wider range of applications. Shen et al.~\cite{shen2020modeling} developed CofeNet, a clinically guided fundus enhancement network that restores retinal structures and removes artifacts from paired high-quality/low-quality fundus images. Li et al.~\cite{li2022annotation} proposed ArcNet, an annotation-free network that utilizes high-frequency components as structural guidance to restore cataract fundus images generated from blurring high-quality fundus images. However, acquiring paired high/low-quality images is challenging in medical settings. The unsupervised method EnlightenGAN~\cite{jiang2021enlightengan} eliminates the dependence on paired training data. CycleGAN~\cite{zhu2017unpaired} introduces cycle consistency constraints to learn the mapping between high-quality and low-quality image domains. StillGAN~\cite{ma2021structure}, an extension of CycleGAN, enhances images by translating low-quality to high-quality domains. It introduces illumination regularization and structure loss, but may suffer from boundary artifacts and difficulties in normalizing illumination distribution.To address these issues, 
% Zhong et al. introduce MAGAN~\cite{zhong2023multi}, a multi-scale attention generative adversarial network designed for unpaired images, which utilizes a feature pyramid and attention distributions to enhance image quality by emphasizing important regions and strengthening constraints on illumination distribution, texture details, semantic features, and smoothness, leading to improved enhancement results.


\subsection{Diffusion-based Generative Models}
Recently, there has been a renewed interest in diffusion-based~\cite{sohl2015deep} and score-matching-based generative models~\cite{hyvarinen2005estimation} due to advancements in denoising diffusion probabilistic models~\cite{ho2020denoising} and noise-conditional score networks~\cite{nichol2021improved, song2019generative}. 
These improvements have led to remarkable capabilities in synthesizing images. 
Both approaches belong to a class of generative models that aim to learn the reverse process of sequentially corrupting data samples with increasing additive noise until the perturbed distribution matches a standard normal prior. 
This is accomplished by optimizing either a time-conditional additive noise estimator~\cite{ho2020denoising} or a noise-conditional score function~\cite{nichol2021improved}, which is the gradient of log-likelihood, parameterized by a deep neural network (DNN). 
These models are then applied in a step-wise denoising process to obtain samples from the data distribution using Langevin dynamics~\cite{welling2011bayesian}. 
It has been demonstrated that denoising diffusion models implicitly learn these score functions at each noise scale, and subsequently, both methods have been reimagined within a unified continuous-time framework based on stochastic differential equations~\cite{song2020score}.

Another perspective that bears a resemblance is the connection between energy-based models and this class of generative methods~\cite{du2019implicit,song2021train}. Energy-based models estimate the unnormalized probability density using the Boltzmann distribution, achieved through the optimization of a DNN that represents the energy function. During testing, one can similarly employ Langevin sampling, starting from pure noise and moving towards the learned distribution, but this time utilizing the gradient of the energy function. It is important to note that energy-based models differ in their training approach, which relies on contrastive divergence methods~\cite{hinton2002training, tieleman2009using}, while diffusion- and score-based models leverage the sequential forward noising (diffusion) scheme to cover a smoother density encompassing isolated modes of the training data distribution.

Recently, diffusion-based conditional generative models have demonstrated state-of-the-art performance across various tasks, including class-conditional data synthesis with classifier guidance~\cite{shi2023exploring}, image super-resolution~\cite{saharia2022image, fei2023generative}, image deblurring~\cite{zhu2023denoising, fei2023generative}, text-based image synthesis~\cite{liu2023more}, and editing~\cite{kawar2023imagic}, as well as general image-to-image translation tasks like inpainting and colorization~\cite{saharia2022palette, anciukevivcius2023renderdiffusion, fei2023generative}. Similar applications of conditional generative modeling can also be observed from a score-based modeling perspective~\cite{chung2022come, meng2021sdedit}. Notably, Kawar et al.~\cite{kawar2022denoising} have recently proposed denoising diffusion restoration models for general linear inverse image restoration problems, which utilize pre-trained denoising diffusion models for unsupervised posterior sampling. However, unlike our model, this approach does not engage in conditional generative modeling and neglects image size agnostic restoration. Furthermore, diffusion models have not been widely explored for image restoration under adverse weather conditions.



==> Sections/abstract.tex <==

\begin{abstract}
The development of medical imaging techniques has significantly contributed to clinical decision-making. However, suboptimal imaging quality, characterized by non-uniform illumination or imbalanced intensity, presents considerable challenges in automating disease screening, analysis, and diagnosis.
Previous GAN-based approaches have been developed for medical image enhancement, eliminating the need for paired images. However, these methods still necessitate training the GAN using a specific dataset to acquire enhancement capabilities, which presents challenges in terms of data collection and training expenses. 
To this end, this paper introduces a training-free Diffusion Model for universal medical image enhancement, named UniMIE. UniMIE does not require any fine-tuning and solely relies on a single pre-trained model from ImageNet to showcase its unsupervised enhancement capabilities across all medical images from various modalities.
Our UniMIE has undergone extensive experimentation across medical image datasets, namely corneal confocal microscopy, retinal color fundus, and endoscopy images. The results of these experiments indicate the superior performance of our method when compared to other low-light enhancement methods. Furthermore, we have conducted an investigation into the effects of our proposed method on various medical image analysis and clinical tasks, including nerve segmentation, tortuosity grading, fovea localization, and disease classification.
\end{abstract}

\begin{IEEEkeywords}
Medical image enhancement, diffusion model, training-free, universal solution.
\end{IEEEkeywords}


==> Table/ablation_bak.tex <==

% \begin{table}[t]
% \setlength{\tabcolsep}{2pt}
% \begin{tabular}{l|ccccc}
% \toprule[1.5pt]
%        & NIQE & PIQE & BRISQUE & AvG & Entropy \\ \midrule[1pt]
% 0.1exp &6.52$\pm$0.69	&87.48$\pm$13.07	&60.80$\pm$7.16	&11.42$\pm$3.08	&6.62$\pm$0.28
% \\
% 0.2exp &6.61$\pm$0.75	&87.96$\pm$12.79	&60.88$\pm$6.78	&11.32$\pm$3.07	&6.56$\pm$0.29
%  \\
% 0.3exp &6.64$\pm$0.74	&85.32$\pm$15.42	&60.72$\pm$6.95	&11.25$\pm$3.06	&6.50$\pm$0.28
% \\
% 0.4exp &6.58$\pm$0.80	&86.11$\pm$15.49	&60.66$\pm$6.06	&11.14$\pm$3.01	&6.44$\pm$0.29
% \\
% 0.6exp &6.52$\pm$0.74	&81.12$\pm$18.80	&59.52$\pm$5.92	&10.92$\pm$2.97	&6.32$\pm$0.30
% \\
% 0.7exp &6.57$\pm$0.72	&84.13$\pm$20.31	&59.37$\pm$6.12	&10.77$\pm$2.95	&6.26$\pm$0.31
%  \\
% 0.8exp &6.71$\pm$0.86	&81.37$\pm$21.42	&58.64$\pm$5.71	&10.59$\pm$2.93	&6.20$\pm$0.32
%  \\
% 0.9exp &6.69$\pm$0.72	&84.44$\pm$18.70    &58.36$\pm$5.21	 &10.46$\pm$0.37	&6.13$\pm$0.34\\ \midrule[1pt]
% DiffMIE   &6.40$\pm$0.69	&84.26$\pm$18.07	&60.07$\pm$6.37	&11.02$\pm$2.99	&6.37$\pm$0.30        \\ \bottomrule[1.5pt]
% \end{tabular}
% \end{table}

% \begin{table}[t]
% \setlength{\tabcolsep}{2pt}
% \begin{tabular}{l|ccccc}
% \toprule[1.5pt]
%             & NIQE & PIQE & BRISQUE & AvG & Entropy \\ \midrule[1pt]
% 0.001       &6.59$\pm$0.76	&87.56$\pm$17.57 &60.38$\pm$7.62 &11.77$\pm$3.13 & 6.39$\pm$0.33\\
% 0.1         & 6.76$\pm$0.87	&82.38$\pm$5.11	&58.04$\pm$6.17 &10.18$\pm$3.28 &6.40$\pm$0.44\\
% 1           &7.00$\pm$1.06	&80.82$\pm$3.12	&57.22$\pm$6.06	&9.74$\pm$3.67	&6.10$\pm$0.59\\
% 10          &6.98$\pm$1.11	&79.59$\pm$3.70	&56.12$\pm$5.46	&9.62$\pm$3.72	&6.06$\pm$0.59
% \\ \midrule[1pt]
% DiffMIE &6.40$\pm$0.69	&84.26$\pm$18.07	&60.07$\pm$6.37	&11.02$\pm$2.99	&6.37$\pm$0.30 \\ \bottomrule[1.5pt]
% \end{tabular}
% \end{table}


==> Table/ablations.tex <==

% \begin{table}[t]\scriptsize
% \setlength{\tabcolsep}{2pt}
% \caption{Ablation Studies on the Combination of Losses.}
% \begin{tabular}{l|ccc|ccccc}
% \toprule[1.5pt]
%      & MSE & EXP & TV & NIQE & PIQE & BRISQUE & AvG & Entropy \\ \midrule[1pt]
% A    & \CheckmarkBold   &     &    &7.03$\pm$0.63	&92.40$\pm$10.13	&59.84$\pm$5.28	&10.34$\pm$2.91	&6.27$\pm$0.32
%  \\
% B    & \CheckmarkBold   & \CheckmarkBold   &    &6.95$\pm$0.68	&90.07$\pm$14.22	&59.03$\pm$6.39	&10.92$\pm$3.00	&6.09$\pm$0.41
% \\
% C    & \CheckmarkBold   &     & \CheckmarkBold  &6.46$\pm$0.65	&85.76$\pm$19.63	&60.87$\pm$7.56	&11.81$\pm$3.13	&6.38$\pm$0.34
% \\ \midrule[1pt]
% DiffMIE & \CheckmarkBold   & \CheckmarkBold   & \CheckmarkBold  &6.40$\pm$0.69	&84.26$\pm$18.07	&60.07$\pm$6.37	&11.02$\pm$2.99	&6.37$\pm$0.30        \\ \bottomrule[1.5pt]
% \end{tabular}
% \end{table}

\begin{table}[t]\scriptsize
\centering
\setlength{\tabcolsep}{3pt}
\caption{Ablation Studies on the Combination of Losses.}
\begin{tabular}{l|ccc|ccccc}
\toprule[1.5pt]
     & MSE & EXP & TV & NIQE & PIQE & BRISQUE & Entropy \\ \midrule[1pt]
A    & \CheckmarkBold   &     &    &7.03$\pm$0.63	&92.40$\pm$10.13	&59.84$\pm$5.28	&6.27$\pm$0.32
 \\
B    & \CheckmarkBold   & \CheckmarkBold   &    &6.95$\pm$0.68	&90.07$\pm$14.22	&\underline{59.03$\pm$6.39}		&6.09$\pm$0.41
\\
C    & \CheckmarkBold   &     & \CheckmarkBold  &\underline{6.46$\pm$0.65}	&\underline{85.76$\pm$19.63} &60.87$\pm$7.56		&\underline{6.38$\pm$0.34}
\\ \midrule[1pt]
\textbf{DiffMIE} & \CheckmarkBold   & \CheckmarkBold   & \CheckmarkBold  &\textbf{4.84$\pm$0.72} &\textbf{47.82$\pm$10.97}	&\textbf{38.43$\pm$4.66}	&\textbf{6.89$\pm$0.27}      \\ \bottomrule[1.5pt]
\end{tabular}
\label{ab:combination}
\end{table}


\begin{table}[t]\scriptsize
\centering
\setlength{\tabcolsep}{1.2pt}
\caption{Ablation Studies on the Weight of Exposure Control Loss.}
\begin{tabular}{l|ccccc}
\toprule[1.5pt]
                &LOE                    &NIQE               &PIQE               &BRISQUE            &Entropy \\ \midrule[1pt]
0.1exp          &761.94$\pm$263.04      &3.67$\pm$0.41	    &\underline{47.87$\pm$8.63}     &39.04$\pm$4.41     &5.98$\pm$0.39\\
0.01exp         &288.72$\pm$123.70      &\textbf{4.84$\pm$0.59}	    &49.55$\pm$9.24     &\underline{38.58$\pm$5.17}     & 6.74$\pm$0.26\\
0.0001exp       &\underline{186.86$\pm$60.21}       &4.91$\pm$0.61	    &48.47$\pm$11.55 	&38.67$\pm$5.13	    & \textbf{6.90$\pm$0.28}\\ \midrule[1pt]
\textbf{DiffMIE (0.001)} &\textbf{186.85$\pm$60.50}       &\underline{4.84$\pm$0.72}	    &\textbf{47.82$\pm$10.97} 	&\textbf{38.43$\pm$4.66}	    & \underline{6.89$\pm$0.27} \\ \bottomrule[1.5pt]
\end{tabular}
\label{ab:exp}
\end{table}


\begin{table}[t]\scriptsize
\centering
\setlength{\tabcolsep}{2pt}
\caption{Ablation Studies on the Well-exposedness Level.}
\begin{tabular}{l|ccccc}
\toprule[1.5pt]
              &LOE                    &NIQE               &PIQE               &BRISQUE            &Entropy \\ \midrule[1pt]
0.1exp        &\textbf{91.79$\pm$48.46}        &5.03$\pm$0.72	  &52.69$\pm$9.97	  &39.38$\pm$3.90	  &\textbf{7.00$\pm$0.27} \\
0.2exp        &\underline{142.52$\pm$73.59}       &\underline{4.88$\pm$0.75}	  &51.00$\pm$8.80	  &38.84$\pm$4.36	  &\underline{6.93$\pm$0.26} \\
0.3exp        &158.75$\pm$98.55       &4.91$\pm$0.59	  &49.99$\pm$8.79	  &38.47$\pm$3.94	  &6.85$\pm$0.26 \\
0.5exp        &375.00$\pm$149.95      &4.93$\pm$0.64	  &50.15$\pm$9.73	  &39.29$\pm$3.53	  &6.63$\pm$0.26 \\
0.6exp        &463.96$\pm$171.14      &4.90$\pm$0.63	  &48.59$\pm$9.50	  &38.82$\pm$4.00	  &6.51$\pm$0.26 \\
0.7exp        &544.19$\pm$187.05      &4.95$\pm$0.60	  &\underline{47.85$\pm$9.76}	  &38.81$\pm$3.47	  &6.40$\pm$0.26 \\
0.8exp        &611.94$\pm$201.35      &4.89$\pm$0.54	  &48.49$\pm$9.30	  &\textbf{38.11$\pm$4.20}	  &6.29$\pm$0.26 \\
0.9exp        &669.80$\pm$213.29      &5.00$\pm$0.52	  &48.20$\pm$9.10     &39.40$\pm$4.13	  &6.19$\pm$0.27 \\ 
\midrule[1pt]
\textbf{DiffMIE (0.4)} &186.85$\pm$60.50      &\textbf{4.84$\pm$0.72}	    &\textbf{47.82$\pm$10.97} 	&\underline{38.43$\pm$4.66}	    & 6.89$\pm$0.27 \\ 
\bottomrule[1.5pt]
\end{tabular}
\label{ab:exp-level}
\end{table}


% \begin{table}[t]
% \setlength{\tabcolsep}{2pt}
% \caption{Ablation Studies on the Weight of Exposure Control Loss.}
% \begin{tabular}{l|ccccc}
% \toprule[1.5pt]
%             & NIQE & PIQE & BRISQUE & AvG & Entropy \\ \midrule[1pt]
% 0.1exp        &3.67$\pm$0.41	&47.87$\pm$8.63    &36.04$\pm$4.41    &17.71$\pm$4.95   &5.98$\pm$0.39\\
% 0.01exp       &4.84$\pm$0.59	&49.55$\pm$9.24     &38.58$\pm$5.17    &16.70$\pm$4.03   & 6.74$\pm$0.26\\
% 0.0001exp     &4.91$\pm$0.61	&48.47$\pm$11.55 	&38.67$\pm$5.13	   &16.94$\pm$4.14	 & 6.90$\pm$0.28\\ \midrule[1pt]
% DiffMIE (0.001) &4.84$\pm$0.72	&47.82$\pm$10.97 	&38.63$\pm$4.66	   &16.87$\pm$4.10	 & 6.89$\pm$0.27 \\ \bottomrule[1.5pt]
% \end{tabular}
% \end{table}




\begin{table}[t]
\centering
\setlength{\tabcolsep}{2pt}
\caption{Ablation Studies on the Weight of Illumination Smoothness Loss.}
\begin{tabular}{l|cccc}
\toprule[1.5pt]
           &LOE & NIQE & PIQE & BRISQUE \\ \midrule[1pt]
0.1        &187.91$\pm$123.47   &4.84$\pm$0.59	&50.05$\pm$10.07    &\underline{38.49$\pm$5.24}   \\
0.01       &187.57$\pm$122.87   &4.85$\pm$0.58	&49.86$\pm$8.19     &38.50$\pm$6.17   \\
1          &\underline{187.55$\pm$123.49}   &4.85$\pm$0.64	&\underline{49.32$\pm$9.35}	    &38.51$\pm$4.93	  \\
10         &187.56$\pm$122.95   &4.86$\pm$0.60	&49.50$\pm$9.89	    &38.61$\pm$5.16	  \\
100        &189.02$\pm$123.99   &4.88$\pm$0.55	&49.48$\pm$9.87   	&38.71$\pm$4.96	  \\
1000       &188.43$\pm$124.09   &4.84$\pm$0.60	&50.42$\pm$9.69   	&38.58$\pm$4.96  \\
10000      &188.16$\pm$123.39   &4.89$\pm$0.58	&49.97$\pm$9.03   	&38.51$\pm$5.07   \\
100000     &187.70$\pm$123.90   &4.87$\pm$0.60	&50.20$\pm$10.99	&38.53$\pm$4.99	  \\
1000000    &188.24$\pm$123.58   &\textbf{4.83$\pm$0.57}	&50.60$\pm$10.89	&38.66$\pm$4.73  \\ \midrule[1pt]
\textbf{DiffMIE (0.001)} &\textbf{186.85$\pm$60.50}       &\underline{4.84$\pm$0.72}	    &\textbf{47.82$\pm$10.97} 	&\textbf{38.43$\pm$4.66}		 \\ \bottomrule[1.5pt]
\end{tabular}
\label{ab:illu}
\end{table}


% \begin{table}[t]
% \setlength{\tabcolsep}{2pt}
% \caption{Ablation Studies on the Guidance Scale.}
% \begin{tabular}{l|ccccc}
% \toprule[1.5pt]
%             & NIQE & PIQE & BRISQUE & AvG & Entropy \\ \midrule[1pt]
% 1e3        &7.96$\pm$0.84	&92.30$\pm$10.079    &48.47$\pm$3.25    &9.31$\pm$3.05   & 5.40$\pm$0.42\\
% 1e4       &5.97$\pm$0.88	&77.76$\pm$18.44     &53.93$\pm$9.13    &16.95$\pm$4.14   & 6.90$\pm$0.28\\ 
% 1e6          &5.79$\pm$2.20 	&29.47$\pm$28.52	    &30.87$\pm$9.01	   &14.85$\pm$7.60	 & 5.16$\pm$2.29
% \\ \midrule[1pt]
% DiffMIE (1e5) &4.88$\pm$0.63	&47.99$\pm$11.15 	&39.04$\pm$4.45	   &16.95$\pm$4.14	 &6.90$\pm$0.28\\ \bottomrule[1.5pt]
% \end{tabular}
% \end{table}



\begin{table}[t]\scriptsize
\centering
\setlength{\tabcolsep}{2pt}
\caption{Ablation Studies on the Guidance Scale.}
\begin{tabular}{l|ccccc}
\toprule[1.5pt]
                &LOE    & NIQE             & PIQE               & BRISQUE           & Entropy \\ \midrule[1pt]
1e3             &815.11$\pm$206.08    &7.96$\pm$0.84	    &92.30$\pm$10.08    &48.47$\pm$3.25     & 5.40$\pm$0.42 \\
1e4             &\underline{376.91$\pm$122.28}   &5.97$\pm$0.88	    &\underline{77.76$\pm$18.44}     &53.93$\pm$9.13     & \textbf{6.90$\pm$0.28} \\ 
1e6             &909.68$\pm$437.70   &\underline{5.79$\pm$2.20} 	&89.47$\pm$28.52	 &\underline{40.87$\pm$9.01}	 & 5.16$\pm$2.29 \\ 
\midrule[1pt]
\textbf{DiffMIE (1e5)}   &\textbf{186.85$\pm$60.50}       &\textbf{4.84$\pm$0.72}	    &\textbf{47.82$\pm$10.97}	&\textbf{38.43$\pm$4.66}	    & \underline{6.89$\pm$0.27}\\ 
\bottomrule[1.5pt]
\end{tabular}
\label{ab:gs}
\end{table}


% \begin{table}[t]
% \setlength{\tabcolsep}{2pt}
% \caption{Ablation Studies on the Well-exposedness Level.}
% \begin{tabular}{l|ccccc}
% \toprule[1.5pt]
%        & NIQE & PIQE & BRISQUE & AvG & Entropy \\ \midrule[1pt]
% 0.1exp  &5.03$\pm$0.72	&52.69$\pm$9.97	  &39.38$\pm$3.90	&15.77$\pm$3.74	&7.00$\pm$0.27
% \\
% 0.2exp  &4.88$\pm$0.75	&51.00$\pm$8.80	  &38.84$\pm$4.36	&16.24$\pm$3.88	&6.93$\pm$0.26
%  \\
% 0.3exp  &4.91$\pm$0.59	&49.99$\pm$8.79	  &38.47$\pm$3.94	&16.52$\pm$3.97	&6.85$\pm$0.26
% \\
% 0.5exp  &4.93$\pm$0.64	&50.15$\pm$9.73	  &39.29$\pm$3.53	&16.78$\pm$4.05	&6.63$\pm$0.26
% \\
% 0.6exp  &4.90$\pm$0.63	&48.59$\pm$9.50	  &38.82$\pm$4.00	&16.81$\pm$4.05	&6.51$\pm$0.26
% \\
% 0.7exp  &4.95$\pm$0.60	&47.85$\pm$9.76	  &38.81$\pm$3.47	&16.79$\pm$4.04	&6.40$\pm$0.26
%  \\
% 0.8exp  &4.89$\pm$0.54	&46.49$\pm$9.30	  &38.11$\pm$4.20	&16.78$\pm$4.02	&6.29$\pm$0.26
%  \\
% 0.9exp  &5.00$\pm$0.52	&46.20$\pm$9.10   &37.40$\pm$4.13	&16.77$\pm$4.00 &6.19$\pm$0.27\\ \midrule[1pt]
% DiffMIE (0.4)   &4.84$\pm$0.59	&49.55$\pm$9.24	  &38.58$\pm$5.17	&16.70$\pm$4.03	&6.74$\pm$0.26
% \\ \bottomrule[1.5pt]
% \end{tabular}
% \end{table}


% \begin{table}[t]
% \setlength{\tabcolsep}{2pt}
% \caption{Ablation Studies on the Well-exposedness Level.}
% \begin{tabular}{l|ccccc}
% \toprule[1.5pt]
%               &LOE                    &NIQE               &PIQE               &BRISQUE            &Entropy \\ \midrule[1pt]
% 0.1exp        &91.79$\pm$48.46        &5.03$\pm$0.72	  &52.69$\pm$9.97	  &39.38$\pm$3.90	  &7.00$\pm$0.27 \\
% 0.2exp        &142.52$\pm$73.59       &4.88$\pm$0.75	  &51.00$\pm$8.80	  &38.84$\pm$4.36	  &6.93$\pm$0.26 \\
% 0.3exp        &158.75$\pm$98.55       &4.91$\pm$0.59	  &49.99$\pm$8.79	  &38.47$\pm$3.94	  &6.85$\pm$0.26 \\
% 0.5exp        &375.00$\pm$149.95      &4.93$\pm$0.64	  &50.15$\pm$9.73	  &39.29$\pm$3.53	  &6.63$\pm$0.26 \\
% 0.6exp        &463.96$\pm$171.14      &4.90$\pm$0.63	  &48.59$\pm$9.50	  &38.82$\pm$4.00	  &6.51$\pm$0.26 \\
% 0.7exp        &544.19$\pm$187.05      &4.95$\pm$0.60	  &47.85$\pm$9.76	  &38.81$\pm$3.47	  &6.40$\pm$0.26 \\
% 0.8exp        &611.94$\pm$201.35      &4.89$\pm$0.54	  &46.49$\pm$9.30	  &38.11$\pm$4.20	  &6.29$\pm$0.26 \\
% 0.9exp        &669.80$\pm$213.29      &5.00$\pm$0.52	  &46.20$\pm$9.10     &37.40$\pm$4.13	  &6.19$\pm$0.27 \\ 
% \midrule[1pt]
% DiffMIE (0.4) &186.85$\pm$60.50       &4.84$\pm$0.72	    &47.82$\pm$10.97 	&38.63$\pm$4.66	    & 6.89$\pm$0.27 \\ 
% \bottomrule[1.5pt]
% \end{tabular}
% \end{table}


==> Table/dataset.tex <==

\begin{table}[t]
\centering
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.0}
\caption{Details information of Selected Datasets.}
\begin{tabular}{l|l|c|c}   
\toprule[1.5pt]
\multicolumn{2}{c|}{\textbf{Datasets}} & \textbf{Dataset Sizes} & \textbf{Image Size} \\ \midrule[1pt]
\multirow{2}{*}{CORN~\cite{corn_dataset}}  
& CORN-1  &580 &\multirow{2}{*}{384$\times$384} \\ 
& CORN-2 &688 &  \\  \hline
\multirow{2}{*}{RFMiD~\cite{pachade2021retinal}} 
& RIADD\_AMD & 131 & \multirow{2}{*}{2144$\times$1424} \\ 
& RIADD\_DR &388  &\\  \hline
CVC-EndoStill~\cite{yin2022duplex}  &Endoscene     &729      &384$\times$288 \\ \hline
\multicolumn{2}{c|}{ISIC2020~\cite{nwoye2020recognition}}
&40       &854$\times$480 \\ \hline
\multicolumn{2}{c|}{CholecT40~\cite{rotemberg2021patient}}  &40       &1920$\times$1080 \\ 
\bottomrule[1.5pt]
\end{tabular}
\label{tab_datasets}
\end{table}






==> Table/dataset_overall.tex <==
\begin{table}[ht]
\centering
\label{tab_datasets}
\caption{The overview of datasets used for evaluating UniMIE.}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule[1.5pt]
Dataset                               & Modality        & Downstream Tasks                      & Number of Selected Scans      &Enhanced image size\\ \midrule[1pt]
CORN~\cite{corn_dataset}              & CCM             & Nerve fibers  segmentation            & 60                &512$\times$512    \\
RIADD~\cite{pachade2021retinal}       & Fundus          & Eye diseases detection                & 192              &512$\times$512    \\
Endoscene~\cite{yin2022duplex}        & Endoscopy       & Polyp segmentation                    & 182               &512$\times$512    \\
ISIC~\cite{rotemberg2021patient}      & Dermoscopy      & Skin cancer segmentation              & 62                &512$\times$512    \\
CholecT40~\cite{nwoye2020recognition} &Endoscopy        & Surgical tools and abdominal tissues  & 56               &512$\times$512    \\
CNCB CT~\cite{zhang2020clinically}    & CT              & Lung,and COVID-19 infection           & 105               &512$\times$512    \\
Brainweb~\cite{Cocosco1997BrainWebOI} & MR-T1, MR-T2, MR-pd     & Brain multiple sclerosis      & 146               &512$\times$512    \\
Hvsmr2016~\cite{Pace2015InteractiveWS} & MRI            & Whole-Heart and Great Vessel          &147                &512$\times$512    \\
DDTI~\cite{pedraza2015open}            & Ultrasound     & Thyroid nodule detection              & 66                &512$\times$512    \\
Kvasir~\cite{Pogorelov2017KVASIRAM}    & Endoscopy      & Polyp segmentation                    & 52                &512$\times$512    \\
NIH Chest X-rays~\cite{wang2017chestx} & CXR            & Pneumothorax segmentation             & 66                &512$\times$512    \\
MSD Hepatic Tumor~\cite{simpson2019large} & CT          & Hepatic tumor  segmentation           & 62               &512$\times$512    \\
Breast Canter~\cite{AlDhabyani2019DatasetOB}  & Ultrasound    &Benign and malignant breast lesion          & 101     &512$\times$512    \\
Nerve Ultrasound~\cite{ultrasound-nerve-segmentation}  & Ultrasound     & Brachial plexus segmentation     & 54     &512$\times$512    \\ \bottomrule[1.5pt]
\end{tabular}
}
\label{tab:dataset}
\end{table}



==> Table/table1.tex <==

%\begin{table}
%\centering
%\caption{SNR (unit: dB) of the Original and Enhanced Corneal Confocal Microscopy Images Using Different Approaches.}
%\label{table}
%\setlength{\tabcolsep}{3pt}
%\scalebox{0.85}{
%\begin{tabular}{l|ccccc}   
%\toprule[1.5pt]
%\multicolumn{1}{c}{Methods} &$r=1$  &$r=3$	&$r=5$	&$r=7$ &$r=9$   \\ 
%\midrule[1pt]
%Original &37.39$\pm$5.41 &32.61$\pm$3.35 &31.08$\pm$3.13 &30.25$\pm$3.25 &29.57$\pm$2.94  \\
%Zero-DCE~\cite{guo2020zero}    &33.94$\pm$5.49  &29.11$\pm$2.44  &28.25$\pm$2.13 &27.81$\pm$2.20  &27.51$\pm$1.97 \\
%Zero-DCE++~\cite{li2021learning}  &34.43$\pm$4.86  &29.19$\pm$2.41  &28.02$\pm$2.26  &27.46$\pm$2.48 &27.00$\pm$2.26  \\
%%%%%%RUAS~\cite{liu2021retinex} &35.72$\pm$9.58  &35.03$\pm$7.23 &41.39$\pm$13.70  &40.10$\pm$9.63 &43.57$\pm$11.50  \\
%SCI~\cite{ma2022toward}  &19.40$\pm$1.44  &21.56$\pm$1.40  &22.80$\pm$1.51  &23.45$\pm$1.62  &23.79$\pm$1.61  \\
%LightenNet~\cite{li2018lightennet}  &31.35$\pm$5.07  &25.64$\pm$3.12  &24.45$\pm$3.18   &24.13$\pm$3.31   &23.84$\pm$3.11 \\
%EnlightNet~\cite{jiang2021enlightengan}  &32.31$\pm$4.80  &25.88$\pm$2.69  &24.61$\pm$2.12   &23.90$\pm$2.39  &23.47$\pm$2.20 \\
%MBLLEN~\cite{lv2018mbllen}  &33.47$\pm$9.66  &26.19$\pm$7.17  &25.78$\pm$8.17 &24.07$\pm$8.76  &22.04$\pm$8.40  \\
%KinD~\cite{zhang2019kindling}        &32.90$\pm$5.38  &25.81$\pm$2.75   &24.01$\pm$2.44   &23.21$\pm$2.46    &22.77$\pm$2.10  \\
%DRBN~\cite{yang2020fidelity}        &35.01$\pm$6.05  &28.06$\pm$3.50  &27.51$\pm$2.72   &27.26$\pm$2.85  &26.83$\pm$2.64 \\
%Retinex-Net~\cite{wei2018deep} &29.73$\pm$5.56   &24.48$\pm$2.16   &23.81$\pm$1.63  &23.46$\pm$1.42   &23.42$\pm$1.30  \\
%TBEFN~\cite{lu2020tbefn}  &25.59$\pm$1.74  &27.56$\pm$1.82  &27.55$\pm$1.95   &27.22$\pm$2.21   &26.96$\pm$2.10 \\
%LiNet~\cite{lore2017llnet}   &33.35$\pm$6.41   &25.59$\pm$4.71   &23.75$\pm$4.35    &22.91$\pm$4.04  &22.25$\pm$3.74 \\
%DSLR~\cite{lim2020dslr}  &32.79$\pm$5.99   &26.56$\pm$3.41   &24.64$\pm$2.97    &23.81$\pm$3.03   &23.23$\pm$2.73  \\ \midrule[1pt]
%%%%%ExCNet~\cite{zhang2019zero}  &32.93$\pm$5.10   &27.21$\pm$2.23   &25.99$\pm$1.97  &25.28$\pm$2.26   &24.88$\pm$2.02 \\
%%%%%%KinD++~\cite{zhang2021beyond}  &29.80$\pm$5.93  &20.15$\pm$1.96  &18.63$\pm$1.48  &18.21$\pm$1.41   &18.14$\pm$1.29  \\ \midrule[1pt]
%\textbf{DiffMIE}  & \textbf{36.00$\pm$5.37}  & \textbf{30.29$\pm$3.17}	& \textbf{28.86$\pm$2.84}	& \textbf{27.98$\pm$2.98}  &\textbf{27.57$\pm$2.76} 
%\\ 
%\bottomrule[1.5pt]
%\end{tabular}}
%\label{Tabel_SNR}
%\end{table} 

\begin{table}[t]\tiny
\centering
\caption{SNR (unit: dB) of the Original and Enhanced Corneal Confocal Microscopy Images Using Different Approaches.}
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|l|ccccc}   
\toprule[1.5pt]
\textbf{Learning}   &\textbf{Methods}   &$\boldsymbol{r=1}$  &$\boldsymbol{r=3}$	&$\boldsymbol{r=5}$	&$\boldsymbol{r=7}$ &$\boldsymbol{r=9}$   \\  \midrule[1pt]
\multirow{8}{*}{Supervised}      
& LLNet~\cite{lore2017llnet}   &33.35$\pm$6.41   &25.59$\pm$4.71   &23.75$\pm$4.35    &22.91$\pm$4.04  &22.25$\pm$3.74 \\
& LightenNet ~\cite{li2018lightennet}  &31.35$\pm$5.07  &25.64$\pm$3.12  &24.45$\pm$3.18   &24.13$\pm$3.31   &23.84$\pm$3.11 \\
& Retinex-Net~\cite{wei2018deep} &29.73$\pm$5.56   &24.48$\pm$2.16   &23.81$\pm$1.63  &23.46$\pm$1.42   &23.42$\pm$1.30 \\
& MBLLEN~\cite{lv2018mbllen}  &33.47$\pm$9.66  &36.19$\pm$7.17  &35.78$\pm$8.17 
&34.07$\pm$8.76  &32.04$\pm$8.40  \\
& KinD~\cite{zhang2019kindling}        &32.90$\pm$5.38  &25.81$\pm$2.75   &24.01$\pm$2.44   &23.21$\pm$2.46    &22.77$\pm$2.10 \\
& KinD++~\cite{zhang2021beyond}  &29.80$\pm$5.93  &20.15$\pm$1.96  &18.63$\pm$1.48  
&18.21$\pm$1.41   &18.14$\pm$1.29  \\ 
& TBFEN~\cite{lu2020tbefn}  &25.59$\pm$1.74  &27.56$\pm$1.82  &27.55$\pm$1.95   
&27.22$\pm$2.21   &26.96$\pm$2.10 \\
& DSLR ~\cite{lim2020dslr}  &32.79$\pm$5.99   &26.56$\pm$3.41   &24.64$\pm$2.97    &23.81$\pm$3.03   &23.23$\pm$2.73 \\ 
\midrule[1pt]
\multirow{2}{*}{Unsupervised} 
& EnlightenGAN ~\cite{jiang2021enlightengan}  &32.31$\pm$4.80  &25.88$\pm$2.69  &24.61$\pm$2.12   &23.90$\pm$2.39  &23.47$\pm$2.20 \\ 
& SCI~\cite{ma2022toward}  &19.40$\pm$1.44  &21.56$\pm$1.40  &22.80$\pm$1.51  &23.45$\pm$1.62  &23.79$\pm$1.61  \\ 
\midrule[1pt]
Semi-supervised  & DRBN~\cite{yang2020fidelity}        &35.01$\pm$6.05  &28.06$\pm$3.50  &27.51$\pm$2.72   &27.26$\pm$2.85  &26.83$\pm$2.64 \\ \midrule[1pt]
\multirow{4}{*}{Zero-shot}     
& Zero-DCE~\cite{guo2020zero}    &33.94$\pm$5.49  &29.11$\pm$2.44  &28.25$\pm$2.13 &27.81$\pm$2.20  &27.51$\pm$1.97 \\
& Zero-DCE++~\cite{li2021learning}  &34.43$\pm$4.86  &29.19$\pm$2.41  &28.02$\pm$2.26  &27.46$\pm$2.48 &27.00$\pm$2.26  \\
& ExCNet~\cite{zhang2019zero}  &32.93$\pm$5.10   &27.21$\pm$2.23   &25.99$\pm$1.97  &25.28$\pm$2.26   &24.88$\pm$2.02 \\ \cline{2-7}
&\textbf{DiffMIE}  & \textbf{36.00$\pm$5.37}  & \textbf{30.29$\pm$3.17}	& \textbf{28.86$\pm$2.84}	& \textbf{27.98$\pm$2.98}  &\textbf{27.57$\pm$2.76} \\  
% \midrule[1pt]
%  &Original &37.39$\pm$5.41 &32.61$\pm$3.35 &31.08$\pm$3.13 &30.25$\pm$3.25 &29.57$\pm$2.94  \\
\bottomrule[1.5pt]
\end{tabular}
\label{Tabel_SNR}
\end{table} 



==> Table/table2.tex <==
% \begin{table}
% \centering
% \caption{High-Quality Score Performance (Mean $\pm$ Standard Deviation) of Different Enhancement Methods.}
% \label{table}
% \setlength{\tabcolsep}{15pt}
% \scalebox{1.0}{
% \begin{tabular}{l|cc}   
% \toprule[1.5pt]
% \multicolumn{1}{c}{Methods} & $s_{HQ}(\text{DR})$   &$s_{HQ}(\text{AMD})$  \\ \midrule[1pt]
% Zero-DCE\cite{guo2020zero}                 &0.5460$\pm$0.4051   &0.3895$\pm$0.3978  \\
% Zero-DCE++\cite{li2021learning}            &0.4956$\pm$0.4014   &0.3828$\pm$0.3980  \\
% SCI\cite{ma2022toward}                     &0.2501$\pm$0.3010   &0.2206$\pm$0.3196  \\
% LightenNet\cite{li2018lightennet}          &0.2861$\pm$0.3935   &0.3449$\pm$0.4346  \\
% EnlightNet\cite{jiang2021enlightengan}     &0.4534$\pm$0.3639   &0.3891$\pm$0.4061  \\
% MBLLEN\cite{lv2018mbllen}                  &0.0851$\pm$0.1433   &0.1436$\pm$0.2500  \\
% KinD\cite{zhang2019kindling}               &0.3884$\pm$0.3555   &0.4312$\pm$0.4121  \\
% DRBN\cite{yang2020fidelity}                &0.2190$\pm$0.3006   &0.2178$\pm$0.3135  \\
% Retinex-Net\cite{wei2018deep}      &\textbf{0.7272$\pm$0.3712}  &\underline{0.5613$\pm$0.4239}  \\
% TBEFN\cite{lu2020tbefn}                    &0.3531$\pm$0.3383   &0.3626$\pm$0.3923  \\
% LiNet\cite{lore2017llnet}                  &0.1922$\pm$0.2802   &0.2537$\pm$0.3548  \\
% DSLR\cite{lim2020dslr}                     &0.2711$\pm$0.3096   &0.3021$\pm$0.3522  \\
% \midrule[1pt]
% \textbf{DiffMIE}                  & \underline{0.6932$\pm$0.3822}   &\textbf{0.5782$\pm$0.4432}  \\ \bottomrule[1.5pt]
% \end{tabular}}
% \label{Table_sHQ}
% \end{table}

\begin{table}[t]
\centering
\caption{High-Quality Score Performance (Mean $\pm$ Standard Deviation) of Different Enhancement Methods.}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{l|l|cc}   
\toprule[1.5pt]
 \textbf{Learning}   &\textbf{Methods}   &\textbf{$\boldsymbol{s_{HQ}}(\text{DR})$}  &\textbf{$\boldsymbol{s_{HQ}}(\text{AMD})$} \\  \midrule[1pt]
\multirow{8}{*}{Supervised}      
& LLNet~\cite{lore2017llnet}                 &0.1922$\pm$0.2802   &0.2537$\pm$0.3548  \\
& LightenNet~\cite{li2018lightennet}   &0.2861$\pm$0.3935   &0.3449$\pm$0.4346  \\
& Retinex-Net~\cite{wei2018deep}      &0.7272$\pm$0.3712  &0.5613$\pm$0.4239  \\
& MBLLEN~\cite{lv2018mbllen}            &0.0851$\pm$0.1433   &0.1436$\pm$0.2500  \\
& KinD~\cite{zhang2019kindling}         &0.3884$\pm$0.3555   &0.4312$\pm$0.4121  \\
& KinD++~\cite{zhang2021beyond}     &0.7052$\pm$0.3452    &0.5665$\pm$0.4320   \\
& TBFEN~\cite{lu2020tbefn}                &0.3531$\pm$0.3383   &0.3626$\pm$0.3923  \\
& DSLR~\cite{lim2020dslr}                   &0.2711$\pm$0.3096   &0.3021$\pm$0.3522  \\ \midrule[1pt]
\multirow{2}{*}{Unsupervised} 
& EnlightenGAN~\cite{jiang2021enlightengan} &0.4534$\pm$0.3639   &0.3891$\pm$0.4061  \\ 
& SCI~\cite{ma2022toward}                 &0.2501$\pm$0.3010   &0.2206$\pm$0.3196  \\  
\midrule[1pt]
Semi-supervised   
& DRBN~\cite{yang2020fidelity}          &0.2190$\pm$0.3006   &0.2178$\pm$0.3135  \\ \midrule[1pt]
\multirow{4}{*}{Zero-shot}       
& Zero-DCE~\cite{guo2020zero}                 &0.5460$\pm$0.4051   &0.3895$\pm$0.3978  \\
& Zero-DCE++~\cite{li2021learning}            &0.4956$\pm$0.4014   &0.3828$\pm$0.3980  \\
& ExCNet~\cite{zhang2019zero}  			&\textbf{0.7747$\pm$0.3399} &\textbf{0.5943$\pm$0.4455}  \\ \cline{2-4}
&\textbf{DiffMIE}  & \underline{0.6932$\pm$0.3822}   &\underline{0.5782$\pm$0.4432}  \\
%\midrule[1pt]
\bottomrule[1.5pt]
\end{tabular}
\label{Table_sHQ}
\end{table}





==> Table/table3.tex <==
% \begin{table*}[htbp]
% \centering
% \caption{SNR (unit: dB) of the Original and Enhanced Corneal Confocal Microscopy Images Using Different Approaches.}
% \setlength{\tabcolsep}{5pt}
% \renewcommand{\arraystretch}{1.05}
% \begin{tabular}{l|l|ccccccc}   
% \toprule[1.5pt]
% \textbf{Learning}   &\textbf{Methods}   & \textbf{LOE$\downarrow$}  &\textbf{PI$\downarrow$}   &\textbf{NIQE$\downarrow$} 	&\textbf{BRISQUE$\downarrow$}	&\textbf{PIQE$\downarrow$}   &\textbf{AvG$\uparrow$}  &\textbf{Entropy$\uparrow$}\\  \midrule[1pt]
% \multirow{8}{*}{supervised learning}      
% & LLNet~\cite{lore2017llnet}  &163.29$\pm$78.31   &7.51$\pm$0.67   &4.28$\pm$0.26  &51.34$\pm$4.75  &63.67$\pm$5.22   &15.92$\pm$3.16  &7.45$\pm$0.14  \\
% & LightenNet~\cite{li2018lightennet}  &554.27$\pm$302.27   &6.08$\pm$0.69   &3.52$\pm$0.40  &37.01$\pm$7.00 &44.68$\pm$8.95  &20.86$\pm$4.09  &7.41$\pm$0.17 \\
% & Retinex-Net~\cite{wei2018deep}  &360.80$\pm$229.81   &5.50$\pm$0.91  &3.67$\pm$0.42  &\textbf{32.43$\pm$7.60}  &41.91$\pm$9.14   &\textbf{23.16$\pm$4.40}   &7.45$\pm$0.29 \\
% & MBLLEN~\cite{lv2018mbllen}  &56.87$\pm$41.04   &8.68$\pm$0.84 &4.89$\pm$0.34  &58.07$\pm$5.14  &65.39$\pm$6.80  &12.92$\pm$3.10   &7.47$\pm$0.16 \\
% & KinD~\cite{zhang2019kindling}  &161.65$\pm$100.35   &6.50$\pm$0.61   &3.99$\pm$0.32  &45.24$\pm$5.21  &53.15$\pm$5.97  &17.56$\pm$3.73   &7.32$\pm$0.21 \\
% & KinD++~\cite{zhang2021beyond}  &244.32$\pm$178.71   &5.76$\pm$0.82  &3.79$\pm$0.50  &38.52$\pm$8.19  &45.37$\pm$9.12   &22.19$\pm$4.98  &7.48$\pm$0.22  \\ 
% & TBFEN~\cite{lu2020tbefn}  &223.43$\pm$117.96   &6.48$\pm$0.49 &3.57$\pm$0.46  &39.68$\pm$6.79  &\textbf{40.97$\pm$10.97}   &17.51$\pm$2.98   &7.38$\pm$0.15 \\
% & DSLR~\cite{lim2020dslr}  &458.23$\pm$274.30   &6.13$\pm$0.50   &3.56$\pm$0.48  &42.66$\pm$5.29  &47.40$\pm$7.50   &21.46$\pm$3.97   &7.39$\pm$0.41 \\ \hline
% Unsupervised learning                 & EnlightenGAN~\cite{jiang2021enlightengan} &803.65$\pm$301.34   & 6.07$\pm$0.72 &3.57$\pm$0.41  &38.74$\pm$5.89  &47.24$\pm$8.47  &20.81$\pm$4.25   &7.53$\pm$0.27 \\ \hline
% \multirow{2}{*}{Self-supervised learning} 
% & DRBN~\cite{yang2020fidelity}   &519.49$\pm$153.12  &6.98$\pm$0.51  &3.94$\pm$0.33  &47.45$\pm$3.74  &60.21$\pm$5.82  &18.29$\pm$3.46  &\textbf{7.60$\pm$0.15}  \\
% & SCI~\cite{ma2022toward}   &407.28$\pm$224.94   &6.07$\pm$0.71   &\textbf{3.46$\pm$0.37} &42.45$\pm$4.55  &49.68$\pm$11.89  &18.78$\pm$4.20   &6.58$\pm$0.49  \\  
% \hline
% \multirow{4}{*}{Zero-shot learning}       
% & Zero-DCE~\cite{guo2020zero}     &343.72$\pm$356.25  & 6.12$\pm$0.63  &3.83$\pm$0.44   &43.23$\pm$6.73  &46.57$\pm$8.10  &18.82$\pm$3.50   &7.24$\pm$0.22\\
% & Zero-DCE++~\cite{li2021learning}  & -  & 6.18$\pm$0.58   &3.64$\pm$0.41  &40.00$\pm$7.27  &47.86$\pm$8.06   &19.01$\pm$3.59  &7.39$\pm$0.20    \\
% & ExCNet~\cite{zhang2019zero}  &717.76$\pm$312.49   
% &5.93$\pm$0.72   &3.66$\pm$0.63  &37.09$\pm$9.73  &33.41$\pm$12.03 &20.00$\pm$3.61   &7.30$\pm$0.22  \\
% &\textbf{DiffMIE (ours)} &\textbf{183.73$\pm$125.44}   &6.63$\pm$0.80     &3.94$\pm$0.34   &39.21$\pm$9.42   &38.66$\pm$21.99    &17.72$\pm$4.44   &\textbf{7.57$\pm$0.16}\\
% %\midrule[1pt]
% \bottomrule[1.5pt]
% \end{tabular}
% \label{Table_noreference}
% \end{table*}



\begin{table}[ht]\scriptsize
\centering
\caption{ Comparison of image quality metrics for different enhancement methods.}
\setlength{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{l|l|ccccccc}   
\toprule[1.5pt]
\textbf{Learning}   &\textbf{Methods}   & \textbf{LOE$\downarrow$}  	&\textbf{BRISQUE$\downarrow$}	&\textbf{PIQE$\downarrow$}    &\textbf{Entropy$\uparrow$}\\  \midrule[1pt]
\multirow{8}{*}{Supervised}      
& LLNet~\cite{lore2017llnet}  &163.29$\pm$78.31     &51.34$\pm$4.75  &63.67$\pm$5.22     &7.45$\pm$0.14  \\
& LightenNet~\cite{li2018lightennet}  &554.27$\pm$302.27     &37.01$\pm$7.00 &44.68$\pm$8.95   &7.41$\pm$0.17 \\
& Retinex-Net~\cite{wei2018deep}  &360.80$\pm$229.81    &32.43$\pm$7.60  &41.91$\pm$9.14      &7.45$\pm$0.29 \\
& MBLLEN~\cite{lv2018mbllen}  &56.87$\pm$41.04     &58.07$\pm$5.14  &65.39$\pm$6.80     &7.47$\pm$0.16 \\
& KinD~\cite{zhang2019kindling}  &161.65$\pm$100.35     &45.24$\pm$5.21  &53.15$\pm$5.97   &7.32$\pm$0.21 \\
& KinD++~\cite{zhang2021beyond}  &244.32$\pm$178.71     &38.52$\pm$8.19  &45.37$\pm$9.12     &7.48$\pm$0.22  \\ 
& TBFEN~\cite{lu2020tbefn}  &223.43$\pm$117.96     &39.68$\pm$6.79  &40.97$\pm$10.97      &7.38$\pm$0.15 \\
& DSLR~\cite{lim2020dslr}  &458.23$\pm$274.30     &42.66$\pm$5.29  &47.40$\pm$7.50     &7.39$\pm$0.41 \\ \hline
\multirow{2}{*}{Unsupervised} 
&EnlightenGAN~\cite{jiang2021enlightengan} &803.65$\pm$301.34     &38.74$\pm$5.89  &47.24$\pm$8.47     &7.53$\pm$0.27 \\
& SCI~\cite{ma2022toward}   &407.28$\pm$224.94    &42.45$\pm$4.55  &49.68$\pm$11.89     &6.58$\pm$0.49  \\  
\hline
Semi-supervised      
& DRBN~\cite{yang2020fidelity}   &519.49$\pm$153.12    &47.45$\pm$3.74  &60.21$\pm$5.82   &7.60$\pm$0.15  \\
\hline
\multirow{4}{*}{Zero-shot}       
& Zero-DCE~\cite{guo2020zero}     &343.72$\pm$356.25     &43.23$\pm$6.73  &46.57$\pm$8.10    &7.24$\pm$0.22 \\
& Zero-DCE++~\cite{li2021learning}  &337.98$\pm$303.22    &40.00$\pm$7.27  &47.86$\pm$8.06     &7.39$\pm$0.20    \\
& ExCNet~\cite{zhang2019zero}  &717.76$\pm$312.49   
  &\textbf{37.09$\pm$9.73}  &33.41$\pm$12.03    &7.30$\pm$0.22  \\
&\textbf{DiffMIE (ours)} &\textbf{183.73$\pm$125.44}      &\underline{39.21$\pm$9.42}       &\textbf{17.72$\pm$4.44}   &\textbf{7.57$\pm$0.16}\\
%\midrule[1pt]
\bottomrule[1.5pt]
\end{tabular}
\label{Table_noreference}
\end{table}
% \vspace{-0.3cm}


==> Table/table4.tex <==
\begin{table*}[htbp]\scriptsize
\centering
\caption{ Segmentation performance of enhanced corneal confocal images using different approaches.}
% \setlength{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l|l|ccccccc}   
\toprule[1.5pt]
\textbf{Learning}   &\textbf{Methods}   &\textbf{Acc}   &\textbf{Sen}   &\textbf{Sp}    &\textbf{Auc}   &\textbf{F1}    &\textbf{IoU}    &\textbf{Dice}\\ \midrule[1pt]
\multirow{8}{*}{Supervised}      
& LLNet~\cite{lore2017llnet}  & 0.9927$\pm$0.0000     & 0.5861$\pm$0.0134  & 0.9967$\pm$0.0000    & 0.9168$\pm$0.0009  & 0.5956$\pm$0.0059  & 0.7104$\pm$0.0014  & 0.7960$\pm$0.0015\\
& LightenNet~\cite{li2018lightennet}  &0.9930$\pm$0.0000     &0.6883$\pm$0.0097 & 0.9959$\pm$0.0000   &0.9493$\pm$0.0007  &0.6439$\pm$0.0058   &0.7361$\pm$0.0015    &0.8202$\pm$0.0014\\
& Retinex-Net~\cite{wei2018deep}  &0.9949$\pm$0.0000    &0.7157$\pm$0.0088  &0.9976$\pm$0.0000     &0.9479$\pm$0.0014  &0.7265$\pm$0.0045   &0.7846$\pm$0.0013    &0.8619$\pm$0.0011\\
& MBLLEN~\cite{lv2018mbllen}  &0.9944$\pm$0.0000     &0.8418$\pm$0.0034  & 0.9959$\pm$0.0000     & 0.9705$\pm$0.0003  &0.7924$\pm$0.0017   &0.7846$\pm$0.0013    &0.8682$\pm$0.0010\\
& KinD~\cite{zhang2019kindling}  &0.9957$\pm$0.0000     &0.7975$\pm$0.0051  &0.9976$\pm$0.0002   &0.9712$\pm$ 0.0002   &0.7784$\pm$0.0027   &0.8179$\pm$0.0011    &0.8881$\pm$0.0007\\
& KinD++~\cite{zhang2021beyond}  &0.9955$\pm$0.0000     &0.7560$\pm$0.0086  &0.9978$\pm$0.0000     &0.9602$\pm$0.0006     &0.7556$\pm$0.0051   &0.8036$\pm$0.0017    &0.8767$\pm$0.0013\\ 
& TBFEN~\cite{lu2020tbefn}  & 0.9950$\pm$0.0000     &0.7977$\pm$0.0038  &0.9969$\pm$0.0000      &0.9690$\pm$0.0002    &0.7485$\pm$0.0022   &0.7976$\pm$0.0008    & 0.8730$\pm$0.0006\\
& DSLR~\cite{lim2020dslr}  &0.9935$\pm$0.0000     &0.6391$\pm$0.0160 &0.9971$\pm$0.0000    &0.9470$\pm$0.0006    &0.6475$\pm$0.0071    &0.7389$\pm$0.0020  &0.8221$\pm$0.0018 \\ \hline
\multirow{2}{*}{Unsupervised} 
&EnlightenGAN~\cite{jiang2021enlightengan} &0.9936$\pm$0.0000      &0.6964$\pm$0.0094  &0.9964$\pm$0.0000   &0.9574$\pm$0.0002      &0.6654$\pm$0.0045   &0.7477$\pm$0.0012    & 0.8310$\pm$0.0011\\
& SCI~\cite{ma2022toward}   &0.9868$\pm$0.0000    &0.0230$\pm$0.0013
&0.9963$\pm$0.0000     &0.6280$\pm$0.0041     &0.0311$\pm$0.0022  &0.5016$\pm$0.0002   &0.5122$\pm$0.0005\\  
\hline
Semi-supervised      
& DRBN~\cite{yang2020fidelity}   &0.9942$\pm$0.0000   &0.7277$\pm$0.0077  &0.9968$\pm$0.0000   &0.9599$\pm$0.0003
    &0.7012$\pm$0.0030   &0.7684$\pm$0.0010    &0.8491$\pm$0.0008\\
\hline
\multirow{4}{*}{Zero-shot}       
& Zero-DCE~\cite{guo2020zero}     &0.9944$\pm$0.0000   &0.7272$\pm$0.0049 &0.9970$\pm$0.0000   &0.9628$\pm$0.0002
    &0.7095$\pm$0.0023   &0.7731$\pm$0.0008    &0.8533$\pm$0.0006\\
& Zero-DCE++~\cite{li2021learning}  &0.9823$\pm$0.0000   & 0.0609$\pm$0.0030 &0.9913$\pm$0.0000  &0.4762$\pm$0.0037  &0.0621$\pm$0.0028 &0.5076$\pm$0.0002   &0.5266$\pm$0.0007  \\
& ExCNet~\cite{zhang2019zero}  &0.9969$\pm$0.0000   
  &0.8983$\pm$0.0026    &0.9979$\pm$0.0000   &0.9828$\pm$0.0002  &0.8454$\pm$0.0018     &0.8656$\pm$0.0009    &0.9219$\pm$0.0005  \\
&\textbf{DiffMIE (ours)} &0.9946$\pm$0.0000      &0.7414$\pm$0.0091  &0.9970$\pm$0.0000     &0.9652$\pm$0.0006  &0.7193$\pm$0.0064   &0.7810$\pm$0.0023  &0.8583$\pm$0.0016 \\

\bottomrule[1.5pt]
\end{tabular}
\label{Table_segmentation}
\end{table*}


==> algo.tex <==
% % !TEX root = ../PaperForReview.tex


\begin{algorithm}[ht]
    \caption{\textbf{UniMIE}}
    \KwIn{Conditioner guided diffusion sampling on $\mathbf{\hat{x}}_{0}$, given a diffusion model $\left(\mu_{\theta}\left(\mathbf{x}_{t}\right), \Sigma_{\theta}\left(\mathbf{x}_{t}\right)\right)$, corrupted image conditioner $\mathbf{y}$, degradation model $\mathcal{D}_{\phi}: \mathbf{y}=f \mathbf{x}+\boldsymbol{\mathcal{M}}$  with randomly initiated parameters $\phi$, guidance scale $s$ for optimizable degradation model. Dictionary of $N$ overlapping patch locations, and a binary patch mask $\mathbf{P}^n$.}
    \KwOut{Output image $\mathbf{x}_{0}$ conditioned on $\mathbf{y}$}

    Sample $\mathbf{x}_{T}$ from $\mathcal{N}(0, \mathbf{I})$
    
    \For{$t$ from $T$ to 1}{

    $\mu, \Sigma = \mu_{\theta}\left(\mathbf{x}_{t}\right), \Sigma_{\theta}\left(\mathbf{x}_{t}\right)$

    $\text {Mean vector 
    }\boldsymbol{\Omega}_t=\mathbf{0} \text { and variance vector } \boldsymbol{\psi}_t=\mathbf{0} \text { and weight vector } \mathbf{G}=\mathbf{0} \text { and } f=\mathbf{0} \text { and } \boldsymbol{\mathcal{M}}=\mathbf{0} $
    
    \For{$k=1,\ldots,K$}{
    $\mathbf{x}_t^{n}=\operatorname{Crop}\left(\mathbf{P}^n \circ \mathbf{x}_t\right) $
    
    $ \mathbf{y}^{n}=\operatorname{Crop}\left(\mathbf{P}^n \circ \mathbf{y}\right) $

    $ \boldsymbol{\mathcal{M}}_{n}=\operatorname{Crop}\left(\mathbf{P}^n \circ \boldsymbol{\mathcal{M}}\right) $

    $\mathbf{\hat{x}}_{0}^{n} =  \frac{\mathbf{x}_{t}^{n}}{\sqrt{\bar{\alpha}_{t}}}-\frac{\sqrt{1-\bar{\alpha}_{t}} \epsilon_{\theta}\left(\mathbf{x}_{t}^{n}, t\right)}{\sqrt{\bar{\alpha}_{t}}}$

    $\mathcal{L}^{total}_{\phi, \mathbf{\hat{x}}_{0}^{n}} = \mathcal{L}(\mathbf{y}^{n}, {\mathcal{D}_\phi}\left(\mathbf{\hat{x}}_{0}^{n}\right)) + \mathcal{Q}\left(\mathbf{\hat{x}}_{0}^{n}\right)$ 

     $f^{n} \leftarrow f^{n} - s \nabla_{f^{n}} \mathcal{L}^{total}_{f^{n}, \mathbf{\hat{x}}_{0}^{n}}$

     $\boldsymbol{\mathcal{M}}^{n} \leftarrow \boldsymbol{\mathcal{M}}^{n} - s \nabla_{\boldsymbol{\mathcal{M}}^{n}} \mathcal{L}^{total}_{\boldsymbol{\mathcal{M}}^{n}, \mathbf{\hat{x}}_{0}^{n}}$

    $\mu^{n} = \mu+s\nabla_{\mathbf{\hat{x}}_{0}^{n}} \mathcal{L}^{total}_{\phi, \mathbf{\hat{x}}_{0}^{n}}$

    $f = f + f^{n}$
    
    $\boldsymbol{\Omega}_t=\mathbf{\Omega}_t+\mathbf{P}^n \cdot \mu^{n} $

    $\boldsymbol{\psi}_t=\boldsymbol{\psi}_t+\mathbf{P}^n \cdot \sigma^n $

    $\boldsymbol{\mathcal{M}} =\boldsymbol{\mathcal{M}} +\mathbf{P}^n \cdot \boldsymbol{\mathcal{M}}^{n} $
    
    $ \mathbf{G}=\mathbf{G}+\mathbf{P}^n$
    
    }
    
    $\mathbf{\Omega}_t=\mathbf{\Omega}_t \oslash \mathbf{G} \quad \quad / / \oslash: \text { element-wise division } $

    $\mathbf{\psi}_t=\mathbf{\psi}_t \oslash \mathbf{G}$

    $\boldsymbol{\mathcal{M}}=\boldsymbol{\mathcal{M}} \oslash \mathbf{G}$

    $f = f/K$
    
    Sample $\mathbf{x}_{t-1}$ by $\mathcal{N}\left(\mathbf{\Omega}_t, \mathbf{\psi}_t \right)$

    }  
    \Return Restored any-size image $\mathbf{x}_0$
\label{algo:patch}
\end{algorithm}

==> algo1.tex <==
% !TEX root = ../PaperForReview.tex

\begin{algorithm}[htbp]
	\caption{\textbf{UniMIE}}
	\KwIn{A a diffusion model $\left(\mu_{\theta}\left(\mathbf{x}_{t}\right), \Sigma_{\theta}\left(\mathbf{x}_{t}\right)\right)$, corrupted image conditioner $\boldsymbol{y}$, gradient scale $s$, degradation model $\mathcal{D}$, distance measure $\mathcal{L}$, optional quality enhancement loss $\mathcal{Q}$, quality enhancement scale $\lambda$.}
	\KwOut{Output image $\mathbf{x}_{0}$ conditioned on $\mathbf{y}$}
        Sample $\mathbf{x}_{T}$ from $\mathcal{N}(0, \mathbf{I})$
        
	\For{$t$ from $T$ to 1}{
	    $\mu, \Sigma = \mu_{\theta}\left(\mathbf{x}_{t}\right), \Sigma_{\theta}\left(\mathbf{x}_{t}\right)$
     
	    $\mathbf{\hat{x}}_{0} =  \frac{\mathbf{x}_{t}}{\sqrt{\bar{\alpha}_{t}}}-\frac{\sqrt{1-\bar{\alpha}_{t}} \epsilon_{\theta}\left(\mathbf{x}_{t}, t\right)}{\sqrt{\bar{\alpha}_{t}}}$
   
        $\mathcal{L}^{total}_{ \mathbf{\hat{x}}_{0}} = \mathcal{L}(\mathbf{y}, {\mathcal{D}}\left(\mathbf{\hat{x}}_{0}\right)) + \lambda \mathcal{Q}\left(\mathbf{\hat{x}}_{0}\right)$ 
  
        $\mathbf{\hat{x}}_{0} \leftarrow \mathbf{\hat{x}}_{0} -s\nabla_{\mathbf{\hat{x}}_{0}} \mathcal{L}^{total}_{ \mathbf{\hat{x}}_{0}}$
    
        Sample $\mathbf{x}_{t-1}$ by $q\left(\mathbf{x}_{t-1} \mid \mathbf{x}_{t}, \mathbf{\hat{x}}_{0}\right) =\mathcal{N}\left(\mathbf{x}_{t-1}; \tilde{\boldsymbol{\mu}}_t\left(\mathbf{x}_{t}, \mathbf{\hat{x}}_{0}\right), \tilde{\beta}_t \mathbf{I}\right)$, 
        
        where $\quad \tilde{\boldsymbol{\mu}}_t\left(\mathbf{x}_{t}, \mathbf{\hat{x}}_{0}\right)=\frac{\sqrt{\bar{\alpha}_{t-1}} \beta_t}{1-\bar{\alpha}_t} \mathbf{\hat{x}}_{0}+\frac{\sqrt{\alpha_t}\left(1-\bar{\alpha}_{t-1}\right)}{1-\bar{\alpha}_t} \mathbf{x}_{t} \quad$ and $\quad \tilde{\beta}_t=\frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_t} \beta_t$
	}
	\Return $\boldsymbol{x}_{0}$
\label{algo6_v1}
\end{algorithm}

